Polyregular Functions

This paper is about certain string-to-string functions, called the polyregular functions. These are like the regular string-to-string functions, except that they can have polynomial (and not just linear) growth. The class has four equivalent definitions: 1. deterministic two-way transducers with pebbles; 2 the smallest class of string-to-string functions that is closed under composition, contains all sequential functions as well as two extra functions called squaring and iterated reverse 3. a fragment of the lambda-calculus, which has a list type constructor and limited forms of iteration such as map but not fold; 4. an imperative programming language, which has for loops that range over input positions. The first definition comes from [milo2003typechecking], while the remaining three are new to the author's best knowledge. The class of polyregular functions contains known classes of string-to-string transducers, such as the sequential, rational, or regular ones, but goes beyond them because of super-linear growth. Polyregular functions have good algorithmic properties, such as: - the output can be computed in linear time (in terms of combined input and output size); - the inverse image of a regular word language is (effectively) regular. We also identify a fragment of polyregular functions, called the first-order polyregular functions, which has additional good properties, e.g. the output can be computed by an AC0 circuit.

==> composition.tex <==

\section{Composition closure for mso interpretations}
First-order string-to-string interpretations are clearly closed under composition; this is essentially by design. 
The goal of this section is to prove Theorem~\ref{thm:composition-mso}, which says that string-to-string \mso interpretations are also closed under composition. For this result it is important that polynomial transductions cannot guess (see Example~\ref{ex:squaring-guessing}) and cannot produce intermediate structures that are not words (see Example~\ref{ex:grids}.

\begin{myexample}\label{ex:squaring-guessing} Define a \emph{nondeterministic position colouring} to be any relation of the form
\begin{align*}
\set{(w,v) \in \Sigma^* \times \Gamma^* : \text{$w$ is obtained from $v$ by applying $f$ to every position}}
\end{align*}
where $f : \Gamma \to \Sigma$ is a fixed function. Define an \emph{nondeterministic \mso string-to-string relation} to be any binary relation obtained by composing some nondeterministic position colouring followed by an \mso string-to-string function. We claim that nondeterministic \mso string-to-string relations are not closed under composition. Indeed, let $f$ be the (deterministic) string to string function which inputs a word $a^n$ over a one letter alphabet and outputs the word $a^{n^2}$ over the same alphabet. Let $R$ be the nondeterministic position colouring which inputs a word of the form $a^m$ and outputs all possible words of the same length over alphabet $\set{a,b}$. If we compose $f$ with $R$, we get the binary relation which inputs a word $a^n$ and outputs all words of length $n^2$ over the alphabet $\set{a,b}$. In particular, for an input of length $n$ there will be exactly $2^{n^2}$ outputs. This relation is not a nondeterministic \mso string-to-string relation, because for a nondeterministic \mso string-to-string relation, the number of outputs on a word of length $n$ is at most $k^n$, where $k$ is some fixed constant.
\end{myexample}

\begin{lemma}\label{lem:forat-decomp}
A string-to-string function is an \mso interpretation if and only if it can be decomposed as first a rational function, then a first-order string-to-string interpretation. In symbols
\begin{align*}
  \msofun = \fofun \circ \ratfun.
\end{align*}
\end{lemma}
\begin{proof}We prove both inclusions separately.
\begin{itemize}
	\item[$\supseteq$] We observe that string-to-string \mso interpretations generalise 
	\item[$\subseteq$] By~\cite[Theorem 2]{Colcombet:2007cm} applied to the special case of words (and not trees), for every alphabet $\Sigma$ and  quantifier rank $k \in \set{1,2,\ldots}$ there exists 
 a letter-to-letter rational transducer 
\begin{align*}
  \xymatrix{\Sigma^* \ar[r]^f & \Gamma^*}
\end{align*}
with the following property. For every
  $n$-ary \mso  query $\varphi$ of quantifier rank $k$ on strings over alphabet $\Sigma$ there exists an $n$-ary first-order query $\psi$ over $\Sigma$ such that 
\begin{align*}
  w \models \varphi(\bar x) \quad \iff \quad f(w) \models \psi(\bar x) \qquad \text{for every }w \in \Sigma^* \text{ and positions $\bar x$ in $w$.}
\end{align*}
Applying this result to the maximal quantifier rank of formulas used in an \mso interpretation, we get the desired result.
\end{itemize}
 \end{proof}


\begin{lemma}\label{lem:swallow-seq} String-to-string \mso interpretations are closed under post-composition with sequential functions
\begin{align*}
  \seqfun \circ \msofun \subseteq \msofun
\end{align*}
\end{lemma}
\begin{proof}

Consider a pebble automaton with states $Q$, which recognises a function
\begin{align*}
  \xymatrix {\Sigma^* \ar[r]^f & \Gamma^*}
\end{align*}



\newcommand{\arity}{\mathsf{ar}}
\begin{claim} Let $h : \Gamma^* \to M$ be a homomorphism into a finite monoid and  let $p,q$ be states of $\Aa$, let $i \in \set{0,1,\ldots}$  and $m \in M$. Then there is an  \mso query of arity $\arity p + \arity q$ with input alphabet $\Sigma$ which selects exactly the tuples
	\begin{align*}
  (w \in \Sigma^*, \bar x \in (\dom w)^{\arity p}, \bar y \in (\dom w)^{\arity q})
\end{align*}
such that   $\Aa$ admits  a run in $w$  from $q \bar x$ to $p \bar y$ which moves only the least significant $i$ pebbles and  produces an output with value $m$ under $h$.
\end{claim}
\begin{proof}
Induction on $i$, in the reverse order, i.e.~the induction base is when $m$ is the number of pebbles in the automaton.
\end{proof}

 For states $q,q'$ of arity $n$ of the pebble automaton, and states $p,p'$ of the DFA, we will define a formula 
 \begin{align*}
  \varphi_{q,q',p,p'}(x_1,\ldots,x_n,y_1,\ldots,y_n)
\end{align*}
selects a tuple $\bar x \bar y$ in a word $w \in \Sigma^*$ if 
which holds if there exists a run of the pebble automaton (and therefore this run is unique) 
\begin{align*}
  (q,\bar x) \to (q
\end{align*}



\end{proof}



\begin{theorem}\label{thm:composition-mso}
	String-to-string \mso interpretations are closed under composition.
\end{theorem}
\begin{proof}
By combining our previous results
\begin{eqnarray*}
	\msofun \circ \msofun & = & \text{(Lemma~\ref{lem:forat-decomp})}\\
	  \fofun \circ \ratfun \circ \msofun  & = & \text{(Elgot and Mezei)}\\
	    \fofun \circ \seqfun \circ \revseqfun \circ \msofun  & \subseteq & \text{(Lemma~\ref{lem:swallow-seq} and its symmetric variant)}\\
	    \fofun \circ  \msofun  & = & \text{(Lemma~\ref{lem:forat-decomp})}\\
	    	    \fofun \circ  \fofun \circ \ratfun  & \subseteq & \text{(Lemma )}\\
	    	    \fofun  \circ \ratfun  & = & \text{(Lemma~\ref{lem:forat-decomp} )}\\ \msofun
\end{eqnarray*}

\end{proof}


==> interpretations-to-pebble.tex <==
\section{From interpretations to pebble transducers}

==> interpretations.tex <==
\section{Interpretations}
In this section, we define first-order and \mso interperations. These are transformations of relational structures that are defined using logical language. In this paper, we care about functional transformations, i.e.~for one input there is at most one output.

\subsection{Logic and interpretations}
\paragraph*{Relational structures and logic.}
A \emph{vocabulary} is a set of \emph{relation names}, each one with associated arity that is a nonnegative integer. 
A \emph{relational structure} over the vocabulary $\Sigma$ consists of a set called the \emph{universe}, and for each relation name in the vocabulary, an associated relation of the same arity over the universe. To define properties of relational structures, we use first-order logic and \mso logic, with the usual syntax and semantics. A transduction with input vocabulary~$\Sigma$ and output vocabulary $\Gamma$ is a set of pairs 
$$\textrm{(input structure over $\Sigma$, output structure over $\Gamma$)}$$ 
which is invariant under isomorphism of relational structures.
Note that a transduction is a relation and not necessarily a function,
thus it can have many different (or zero) possible outputs for the same input. A transduction is called functional if it is a partial function, i.e.~for every input there is at most one output up to isomorphism.




\paragraph*{Generalised arities.} The idea behind an interpretation is that it inputs a relational structure, and outputs a new one, where the elements of the output structure are coded in tuples of elements of the input structure. In some cases, it is enough to fix a dimension, say 3, and have code elements of an output structure as 3-tuples of elements of the input structure. In other cases, it is more convenient to use copying and varying dimensions, e.g.~elements of the output structure are going to be coded in 2 copies of the input structure plus one 3 copies square of the input structure. To account for such copying, we use powers $X^n$ where is $n$ is not necessarily a natural number, but a ranked set as described below.


A \emph{ranked set} is a set where each element has an associated arity, e.g.~the vocabulary for a relational structure is a ranked set. For a ranked set $Q$ and set (not ranked $X$), define
\begin{align*}
X^Q = \set{q(x_1,\ldots,x_n) : \text{$q \in Q$ has arity $n$ and }x_1,\ldots,x_n \in X}.
\end{align*}


  If $P,Q$ are ranked sets, then their product $P \times Q$ is defined as the usual product, with the arity of a pair $(p,q)$ being  the sum of arities of its components $p$ and $q$.
This power operation generalises the usual power $\structa^n$ for $n \in \set{0,1,2,\ldots}$, by viewing $n$ as a ranked set which has one element of arity $n$.  The generalised notion of arity will be useful for us because it avoids a certain amount of coding in interpretations.

\paragraph*{Queries and interpretations.} 
For a ranked set $Q$, define  a \emph{$Q$-ary query over input signature $\Sigma$} to be any function $\varphi$ of the form
\begin{align*}
\structa \in \text{relational structures over $\Sigma$} \qquad \mapsto \qquad 	\varphi(\structa) \subseteq \structa^Q.
\end{align*}
We say that the query is definable in \mso (respectively, first-order logic) if for every $q \in Q$ of rank $n$ there is a formula $\varphi_q$ of \mso (respectively, of first-order logic)  with $n$ free first-order variables such that 
\begin{align*}
\structa,a_1,\ldots,a_n \models \varphi_q \quad \iff \quad (q,a_1,\ldots,a_n) \in \varphi(\structa) 
\end{align*}
holds for every structure $\structa$ and $a_1,\ldots,a_n$ in its universe. Note that even when talking about \mso queries, which can use quantification over sets, the free variables are still first-order variables.




\begin{definition}[Interpretation]
The syntax of a  \emph{first-order (respectively, \mso) interpretation} consists of:
	\begin{itemize}
		\item an input vocabulary $\Sigma$ and an output vocabulary $\Gamma$;
		\item a finite ranked set $Q$;
		\item a first-order (respectively, \mso)  $Q$-ary query over the input vocabulary called the \emph{domain query};
		\item for each $n$-ary relation $R$ of the output vocabulary, a first-order (respectively, \mso) $Q^n$-ary query $\varphi_R$ over vocabulary $\Sigma$ (for the definition of $Q^n$, recall the definition of products for ranked sets).
	\end{itemize}
The \emph{dimension} of the interpretation is the highest arity appearing in $Q$.
\end{definition}
	If $\Ii$ is an interpretation (first-order or \mso) and $\structa$ is a relational structure over the input vocabulary then $I(\structa)$ is defined to be the structure over the output vocabulary where:
	\begin{itemize}
		\item the universe is the value of the domain query on $\structa$;
		\item each relation $R$ is interpreted as $\varphi_R(\structa)$ interested with the domain.
	\end{itemize}
We view the semantics of an interpretation, i.e.~the mapping $\structa \mapsto I(\structa)$ as a transduction, i.e.~we only care about the isomorphism type of the input and output.  Therefore, two interpretations are considered equal if for every input structure, the outputs of both interpretations are isomorphic.

The above definition is essentially the same as the classical notion of interpretation, see~\cite[Section 5.3]{Hodges:1993ki}. The only difference is that we use the generalised notion of arity, which means that some elements of the output structure can be interpreted as triples, and some as pairs, etc. In classical model theory, one is typically interested in interpreting one infinite structure in another and therefore generalised arities do not contribute any new expressive power since they can be coded inside tuples of a common but higher dimension. In this paper we are more interested in an interpretation as giving a function from (typically finite) structures to other ones. From this viewpoint, the generalised notion of arity is useful, e.g.~if the input structure has a universe of size one, then generalised (but not usual) arities still allow the output to have size greater than one. 


\paragraph*{Composition.}
First-order interpretations are closed under composition~\cite[p.~218]{Hodges:1993ki}. The proof is by simply inlining the formulas of the first interpretation inside the formulas of the second interpretations. This method does not work 
for \mso interpretations in general. To see the problems with composition, suppose that we want to compose two \mso interpretations
\begin{align*}
  \xymatrix{\text{structures over $\Sigma$} \ar[r]^I  & \text{structures  over $\Gamma$} \ar[r]^J & \text{structures over $\Delta$}}
\end{align*}
The \mso formulas used by the second interpretation  quantify over sets of elements produced by the first interpretation. Since elements produced by the first interpretation are tuples of elements in the original input, the natural way to compose the two interpretations would require quantifying over sets of tuples in the input structure.  We will see counterexamples in Section~\ref{sec:successor-bad-idea}.


\subsection{String-to-string interpretations}
Our goal is to use \mso interpretations and \fo interpretations to transform strings into strings. It is important to define how strings are represented as relational structures, so that we can evaluate the formulas used in interpretations. The long and short is that we represent strings using the ordering on positions, and not just the successor relation. This choice is important for both \fo interpretations (because an \fo formula cannot reconstruct the order on the input positions when it has only the successor) and for \mso interpretations (because it is harder, even for \mso, to produce the order on output positions instead of the successor).  Since the distinction between order and successor is crucial to this paper, the definitions below are given with more formal notation than elsewhere in the paper. 
 
Let $\Sigma$ be a finite set. Define $\ordstruct \Sigma$ to be structures over a vocabulary with one binary relation $<$ and one unary relation $a(x)$ for each element of $\Sigma$, modulo isomorphism of relational structures.  We view a  word $w \in \Sigma^*$ as a structure $\underline w$ over the vocabulary described above in the following way: the universe of $w$ is the set of positions, the relation $<$ represents the order on positions, and the each predicate $a(x)$ selects positions with label $a$.  


\begin{definition}\label{def:string-to-string-mso-interpretations}
	A \emph{string-to-string \mso  (respectively, \fo) interpretation}  is a function
\begin{align*}
  f : \Sigma^* \to \Gamma^*,
\end{align*}
	where $\Sigma$ and $\Gamma$ are finite alphabets, such that there exists an \mso  (respectively, \fo) interpretation $I$ which makes the following diagram commute
\begin{align*}
  \xymatrix{
  \Sigma^* \ar[r]^f \ar[d]_{w \mapsto \underline w} & \Gamma^* \ar[d]^{w \mapsto \underline w} \\
  \ordstruct{\Sigma} \ar[r]_I & \ordstruct{\Gamma}
  }
\end{align*}
\end{definition}
In Section~\ref{sec:successor-bad-idea}, we explain why we use the order $<$ and not the successor. 


\subsection{Why successor is a bad idea}
\label{sec:successor-bad-idea}
\newcommand{\succode}[1]{\underline{\underline{#1}}}
Consider an alternative definition of string-to-string \mso interpretations, which uses successor instead of order. The goal of this example is to show that this is a bad idea. For a finite alphabet $\Sigma$, consider the encoding of words as relational structures
\begin{align*}
  \xymatrix@C=3cm{ \Sigma^* \ar[r]^{w \mapsto \succode w} & \sucstruct \Sigma},
\end{align*}
which is defined the same way as $\underline w$, but  the structures are equipped with  binary successor relation
\begin{align*}
  x = y+1
\end{align*}
instead of the order $x < y$. Define $X_{mso}$ (respectively, $X_{fo}$)  to be the class of functions  $f : \Sigma^* \to \Gamma^*$  which satisfy the conditions from Definition~\ref{def:string-to-string-mso-interpretations} (using the logics \mso and \fo, respectively) except that the encoding $\succode w$ used instead of $\underline w$.  We claim that
\begin{enumerate}
	\item the class $X_{mso}$ is a strict superset of the string-to-string \mso transductions;
	\item the class $X_{fo}$ is incomparable to the class of string-to-string \fo transductions;
	\item neither of the classes $X_{mso}$ and $X_{fo}$ is closed under compositions;
	\item 
\end{enumerate}


\begin{myexample}[Folklore]\label{ex:grids}
We show two \mso interpretations $I$ and $J$ whose composition is not an \mso interpretation. In this example, $I$ is actually a first-order interpretation, and $J$ is an \mso formula, which can be viewed as a special case of an \mso interpretation which produces only two output structures, representing ``true'' and ``false''. 
Consider the following two \mso transductions (which are partial functions, i.e.~for every input structure there is at most one output structure):
\begin{enumerate}
\item  Let us view a word $ w \in \set{\red \bullet, \blue \bullet}^*$ as a relational structure, where the universe is positions, there are unary predicates for ``has label $\red \bullet$'' and ``has label $\blue \bullet$'', as well as a binary predicate for the successor relation, as in the following picture:
\mypic{1}
Let $\Ii$ be the transformation  which inputs a structure over the vocabulary above, assuming that it is indeed an representation of a word, and which 
 outputs a directed graph with nodes coloured by $\set{\red \bullet, \blue \bullet}$   like this:
\mypic{2}
For this example, it is not important what the interpretation does for inputs that do not represent words. It is easy to implement such a transformation using an \mso (in fact, first-order) interpretation of dimension two.
\item Fix some deterministic Turing machine $M$. We code a computation of $M$ as a labelled grid as in the following picture:

 Let $\Jj_M$ be the transduction which inputs an $n \times k$ grid with the first row is labelled by a configuration of $M$, and which outputs the same grid with the $i$-th row containing the $i$-th configuration of the machine in its computation (assuming the first configuration is as given in the input). 
	
\end{enumerate}

\end{myexample}

Because of the problem with composition described above,  one typically studies \mso interpretations of dimension 1, which are closed under composition in the natural way~\cite[Theorem 7.14]{Courcelle:2012wq}. For \mso interpretations of dimension higher than 1, closure under composition no longer holds, as shown in the following example.




==> mso-equivalence.tex <==
\section{Reduction to first-order}
\label{sec:reduction-to-first-order}



The following result follows from~\cite[Theorem 2]{Colcombet:2007cm} applied to the special case of words (and not trees), see also~\cite[Theorem 3.2]{Kazana:2013jq}.
 
 \begin{lemma}\label{lem:rat-decomp} Every \mso query over words can be decomposed as first a letter-to-letter rational function, and then a first-order query. In a diagram:
\begin{align*}
\forall \red \exists \qquad 
  \xymatrix@C3cm{
  \Sigma^* \ar@[red][rr]^{\red f}_{\red{\text{letter-to-letter }\ratfun}} \ar[dr]^\varphi_{\text{\mso}}  & & \red{\Gamma^*} \ar@[red][dl]_{\red{\psi}}^{\red{\text{\fo}}} \\ & \mathsf{P}(\set{1,2,\ldots}^n)
  }
\end{align*}


\end{lemma}
\begin{proof}
\end{proof}



\begin{align*}
  \msopebfun \subseteq \fopebfun \circ \ratfun \subseteq \foprogfun \circ \ratfun \subseteq \msoprogfun 
\end{align*}


\begin{align*}
  \msoprogfun \subseteq \msointfun
\end{align*}


\begin{align*}
  \msointfun \subseteq \fointfun \circ \ratfun \subseteq \foprogfun \circ \ratfun \subseteq \msopebfun \circ \msopebfun
\end{align*}



==> nested-to-program.tex <==
\section{From nested two-way transducers to programs}



For nested pebble automaton $\Aa$ and a control state $q$ of the root automaton in $\Aa$, define 
\begin{align*}
\tau q\Aa \sigma : \Sigma^* \to (\Gamma + \bigcup_{\Bb} \bigcup_{q \in \mathsf{states}\Bb} \set{q\Bb,\Bb q} )^*	
\end{align*}


\begin{definition}
	A set $X$ of nested two-way automata (with the same input alphabet $\Sigma$ but possibly different and output alphabets) is called \emph{compositional} if there exists a monoid homomorphism
\begin{align*}
  h : \Sigma^* \to M
\end{align*}
	such that
	for every $\Aa \in X$ and every $m_1,m_2$ there exists a substitution term $t$ with variables $X \times \set{1,2}$ such that
	\begin{align*}
  \Aa(w_1 w_2) = t[ (\Bb,i) \mapsto \Bb(w_i)] \qquad \text{for every $w_1,w_2 \in \Sigma^*$ with $h(w_i)=m_i$}
\end{align*}
\end{definition}


\begin{lemma}\label{lem:}
For every nested two-way automaton  of order $k$ there exists a finite compositional set of nested two-way automata of order $\le k$ that contains it.
\end{lemma}
\begin{proof}
Induction on the order $k$.
\end{proof}


\begin{lemma}\label{lem:}
Let $X$ be a set of nested two-way automata that is compositional, as witnessed by a homomorphism $h : \Sigma^* \to M$.  There exists a program
\begin{align*}
  \Sigma^* \to \prod_{\Aa \in X} (\text{output alphabet of }\Aa)^*
\end{align*}

\end{lemma}
\begin{proof}
\end{proof}



==> nested-to-streaming.tex <==
\section{From nested two-way transducers to polynomial streaming transducers}



\begin{lemma}
  Let $\Aa$ be a nested two-way transducer of order $k$. There exists a finite set $X$ of nested two-way transducers of orders $<k$ with the following property.
\end{lemma}
\begin{proof}
\end{proof}

If $X \subseteq \set{1,\ldots,k}$ is a subset of the pebbles, define a pebbled word to be a word in $\Sigma^*$ together with a \emph{pebbling}, which is  a partial function
\begin{align*}
\set{1,\ldots,k} \to \dom w
\end{align*}
which says where the pebbles are placed (some are not placed at all). Input words can be seen as a special case of pebbled words where pebbling is completely undefined. On pebble words we define a partial concatenation operation, which is defined only when the the pebblings of the concatenated pebbled words have disjoint domains.


\paragraph*{Types of pebbled words.}
For a pebbling $w$ we define its \emph{type} to be its first-order type of appropriate quantifier rank with respect to the automaton.  We write $\tau,\sigma$ for types of pebbled words. By compositionality, the set of types can be equipped with a partial associative operation such that the function which maps $\tp$ a pebbled word to its  type is a homomorphism of partial semigroups, i.e.~for every pebbled words $w,v$, the values
\begin{align*}
\tp(wv) \qquad  \tp(w) \cdot \tp(v)
\end{align*}
are either both undefined or both defined and equal. We view pebbled words as acting on types, i.e.~if $\tau$ is an type, say of some pebbled word $w$, and $u,v$ are pebbled words, then we define $u \tau v$ to be the type of the pebbled word $uwv$; this does not depend on the choice of $w$.



\paragraph*{The tree structure of configurations.}
Let $q$ be a state of the pebble automaton with rank $i$, and let $w$ be a pebbled word where the pebbles used are $\set{1,\ldots,i}$. Then we write $q(w)$ for the corresponding configuration of the automaton, which has control state $q$ and pebbles in the positions indicated by the pebbling of $w$.  For pebbled words $u,v,w$ such that $uvw$ is defined and has $i$ pebbles, define
\begin{align*}
\conft uvw 
\end{align*}
to be the set of configurations $c$ which extend the pebbling $uvw$, and such that pebble $i+1$ is in the word $v$. The set $\conft uvw$ can be viewed as an ordered forest. Define 
\begin{align*}
\borderconf u v w \subseteq \conft uvw
\end{align*}
to be the roots of this forest which are either first or last roots of the forest. 

Fix some total ordering on the control states of the automaton. Using this ordering, we can define a total ordering on the configurations in a given word, where the configurations are first ordered based on the control states, and then lexicographically based on their pebble positions.  For a set of configurations $X$ and  $i \in \set{1,2,\ldots}$ define $X[i]$ to be the $i$-th element of $X$ in the above defined ordering. This element is undefined if $|X|<i$.

Define 
\begin{align*}
\out i uvw  \in  \Sigma^*	
\end{align*}
as follows. Let $c$ be the $i$-th configuration in $\firstconf u v w$ in lexicographic ordering. Consider the run of the pebble automaton which starts in configuration $c$, and let $d$ be the first configuration from $\lastconf u v w$ that appears in this run. (If $c \in \lastconf u v w$, then $c = d$).  
\begin{lemma}
  The number of elements in $\firstconf  u v w$ depends only on the types of $u,v,w$.
\end{lemma}
\begin{proof}
\end{proof}


\begin{align*}
\out i \tau v \sigma \in (\Sigma + X)^* \qquad 	
\end{align*}



Motivated by the above lemma, we can write 
\begin{align*}
\firstconf \tau \pi \sigma \in \set{0,1,2,\ldots}
\end{align*}
 to represent the number of elements in $\firstconf  u v w$, for $u,v,w$ being pebbled words of types $\tau,\pi,\sigma$.  Define
\begin{align*}
\out i \tau w \sigma :  \pwords_\tau \to \pwords_\sigma  \to  \Sigma^* 
\end{align*}
to be the function defined by
\begin{align*}
\lambda u \in \pwords_\tau.\ 	\lambda v \in \pwords_\sigma.\ 	
\end{align*}


\begin{lemma}
  There is a register automaton which maps 
\end{lemma}
\begin{proof}
\end{proof}



\begin{lemma}
  Let $\tau, \pi, \sigma$ be types such that $\tau \pi \sigma$ is defined. To each pebbled word $w$ of type $\pi$ one can associate a term $\termik \tau w \sigma$ with the following properties:
  \begin{enumerate}
  	\item the term depends only on $w$ and the types of $u,w$; 
  	\item the type of the term depends only on the types of $u,v,w$;
  	\item Let $u,v$ be pebbled words of types $\tau,\sigma$ respectively. Then
\begin{align*}
\out i u v w = (\termik u v w) (\termik \varepsilon u  {vw}) (\termik {uv} w  \varepsilon)
\end{align*}

  \end{enumerate}
\end{lemma}
\begin{proof}
\end{proof}


\begin{lemma}\label{lem:letter}
  Let $\tau,\pi,\sigma$ be types such that the type $\tau \pi \sigma$ is defined, and let 
  \begin{align*}
i \in \borderconf \tau \pi \sigma.
\end{align*}
There exists a function
\begin{align*}
f :  \pwords_\pi  \to  (\Gamma + \vars \tau \pi \sigma)^*
\end{align*}
with the following properties
\begin{enumerate}
	\item for every pebbled words $u,v,w$ of types $\sigma,\tau$ respectively, 
\begin{align*}
\out i u v w 
\end{align*}
is obtained by applying to the word $f(v)$ the subsitution
\begin{align*}
(\pi,j) \mapsto \out j \pi w \varepsilon	 \qquad (j,\pi) \mapsto \out j \pi w \varepsilon	
\end{align*}
\item if $\pi$ has no pebbles then $f$ is computed by a register automaton.
\end{enumerate}
\end{lemma}



\begin{lemma}\label{lem:letter}
  Let $\tau,\sigma$ be be types and let $a$ be a pebbled word of length one such that the type $\tau a \sigma$ is defined, and let 
  \begin{align*}
i \in \borderconf \tau a \sigma.
\end{align*}
Then there is a word 
  \begin{align*}
\out i \tau a \sigma	  \in (\Gamma + X)^*
\end{align*}
such that for every pebbled words $u,w$ of types $\sigma,\tau$ respectively, 
\begin{align*}
\out i u a w = \eta(\out i \tau a \sigma)
\end{align*}
holds where $\eta$ is the subsitution
\begin{align*}
(\pi,j) \mapsto \out j \pi w \varepsilon	 \qquad (j,\pi) \mapsto \out j \pi w \varepsilon	
\end{align*}

\end{lemma}
\begin{proof} Induction on the number of pebbles in the type $\tau a \sigma$, in the opposite order, i.e.~the induction base is that there are $k$ pebbles and the the induction step goes from $k$ to $k-1$. 

\begin{itemize}
	\item \emph{Induction base.} In the induction base, all pebbles are present in the configuration, and  therefore 
\begin{align*}
\borderconf \tau a \sigma
\end{align*}
is empty 
and there are no $i$ to consider.
\item \emph{Induction step.} Let $\tau, \sigma, a$ and $i$ be as in the assumption of the lemma. Suppose that we are given pebbled words $u,v$ of types $\tau$ and $\sigma$ respectively. Our goal is to produce, using a term, the function
\begin{align*}
\out i u a v	 
\end{align*}
Suppose that the number of pebbles in $uav$ is $k-1$, and let 
\begin{align*}
q_1,\ldots,q_m	
\end{align*}
be all the states of rank $k$, listed in according to our fixed ordering on control states. Then the $i$-th element of   $\borderconf u a v$ is
\begin{align*}
q_i(u{\stackrel {k} a}v).
\end{align*}
The successor configuration of the above is 

\begin{align*}
\out i u a v = \out j \varepsilon {u{\stackrel {k} a}v} \varepsilon 	
\end{align*}
By Lemma ...
\begin{align*}
	\out j \varepsilon {u{\stackrel {k} a}v} \varepsilon 	
\end{align*}

\begin{align*}
		\out j \varepsilon {u} {\stackrel {k} a v}  \qquad 		\out j  {u \stackrel {k} a}  v \varepsilon
\end{align*}


Suppose that $\pi_i$ is the type of $\stackrel k a$. By induction assumption, 
we have terms
\begin{align*}
\out i u {\pi_i} \sigma \qquad \out i \tau {\pi_i} v
\end{align*}








\end{itemize}
\end{proof}


\begin{lemma}\label{lem:binary}
  Let $\tau,\pi_1,\pi_2,\sigma$ be types of pebblings such that the type $\tau 
  \pi_1 \pi_2 \sigma$ is defined. Then there is a term $M$ such that
  \begin{align*}
\out i \tau {w_1w_2} \sigma  = M \out i \tau {w_1} {w_2 \sigma} \out i {\tau w_1} {w_2} \sigma
\end{align*}
holds for every pebbled words $w_1,w_2$ of types $\pi_1,\pi_2$ respectively.
\end{lemma}
\begin{proof}
Induction on the number of pebbles used in the type $\tau \pi_1 \pi_2 \sigma$, with the base case being 
\end{proof}


\begin{lemma}\label{lem:unranked}
  Let $\tau,\pi,\sigma$ be types of pebblings such that the type $\tau 
  \pi_1 \pi \sigma$ is defined and $\pi$ has no pebbles. Then there is a term $M$ such that
  \begin{align*}
\out i \tau {w_1 \cdots w_n} \sigma  = M [M_1,\ldots,M_n] \qquad \text{where} M_i =  \out i {\tau w_1 \cdots w_{i-1}} {w_i} {w_{i+1} \cdots w_n \sigma}
\end{align*}
holds for every $n$ and every pebbled words $w_1,\ldots,w_n$ of type $\pi$.
\end{lemma}
\begin{proof}
\end{proof}





==> nested.tex <==
\section{Nested two-way transducers}


\begin{definition} [Nested two-way transducer] \label{def:nested-two-way} Let $k \in \set{1,2,\ldots}$. 
The syntax of   \emph{nested two-way transducer of order $k$}   consists of:
\begin{itemize}
\item input and output alphabets $\Sigma$ and $\Gamma$;
	\item a deterministic two-way automaton with input alphabet $\Sigma$, called the \emph{root automaton};
	\item a finite set of nested two-way automata of order $<k$, called the \emph{child automata}, where the input and output alphabets are also $\Sigma$ and $\Gamma$;
	\item an 
output function from the states of the root automaton to
\begin{align*}
(\Sigma + \text{child automata} \times \set{\text{left, right}})^*
\end{align*}
\end{itemize}	
\end{definition}

For a nested two-way transducer $\Aa$, its semantics is the function
\begin{align*}
  \sem \Aa : \Sigma^* \to \Gamma^* 
\end{align*}
defined as follows by induction on the order. Let $w \in \Sigma^*$ be an input word, and consider the run of the root automaton over $w$, which is a sequence 
\begin{align*}
  (q_1,x_1),\ldots,(q_n,x_n)
\end{align*}
of pairs of the form (state of the root automaton, position in the input word). For each $i \in \set{1,\ldots,n}$, the output produced in the $i$-th configuration is defined as follows. If $x_i$ is one of the end markers $\vdash$ or $\dashv$, then no output is produced (i.e.~the empty word is produced). Otherwise, the output produced in the $i$-th configuration is defined as follows. Decompose the input  as follows:
\begin{center}
	picture
\end{center}
Apply the output function of the automaton to the state $q_i$, yielding some word 
\begin{align*}
v_i \in (\Sigma + \text{child automata} \times \set{\text{left, right}})^*
\end{align*}
For each child automaton $\Bb$, in the word $v_i$ replace the letter $(\Bb,\mathrm{left})$ by the output produced by $\Bb$ on the left word, likewise for right. The resulting word is the output produced in the $i$-th configuration. The output of $\Aa$ is then defined by concatenating, in left-to-right order, the outputs produced in all the configurations.


A nested two-way transducer is called \emph{first-order definable} if the root automaton, the child automata, their child automata, and so on, are all first-order definable.







==> pushdown-to-program.tex <==
\section{From pushdowns to programs}

\begin{lemma}\label{lem:pushdowns-to-programs}
 If a function $f : \Sigma^* \to \Gamma^*$  is computed by a  first-order pushdown machine, then it is computed by a first-order polynomial program.
\end{lemma}



%\begin{lemma}\label{lem:linear-interpret}
%  Let $\Sigma, \Gamma$ be finite sets, let $k \in \Nat$ and let 
%    \begin{align*}
%I : \Sigma^* \to \terms 	\Gamma^*
%\end{align*}
%be a linear first-order interpretation that produces only terms of depth at most $k$.  Then the function which maps $w \in \Sigma^*$ to the value of the term $I(w)$ is a polynomial first-order program.
%\end{lemma} 
%\begin{proof} By~\cite{}, the function which maps $w \in \Sigma^*$ to the syntax tree of the term $I(w)$ is (even linear) first-order list program. The output $I(w)$ can then be interpreted by a polynomial first-order list program.
%\end{proof}
%


\begin{proof}
Let $\Aa$ be a first-order pushdown machine. The computation of $\Aa$ on a word $w$ looks like this:
\mypic{8}
The sequence of pushdown operations during the computation can be organised into a bounded depth tree,  with nodes labelled by operations of the machine $\Aa$,  as in the following picture
\mypic{9}
The bounded depth tree can be produced be linear first-order list program, thanks to~\cite{}. 
\end{proof}


==> streaming-to-program.tex <==
\section{From streaming transducers to programs}




\begin{lemma} Let $r$ be a register of $\Aa$, and let $\Sigma_r$ be the alphabet of $r$. Then there is a polynomial list  program
  \begin{align*}
M : O^* \to (\Sigma_r)^*
\end{align*}
which maps a sequence $w$ of register operations to the value of register $r$ after performing all of these operations.
\end{lemma}
\begin{proof}
Induction on the position of $r$ in the order on registers.
\end{proof}


==> streaming.tex <==
\section{Polynomial streaming transducers}
In this section we define polynomial streaming (string-to-string) transducers. The transducer reads its input from left to right (but using regular lookahead). It has a fixed number of registers, store parts of the output word. 
Before 

\begin{myexample}[Running example] Here is a polynomial streaming transducer which recognises the function
\begin{align*}
w \in \set{a,b}^* \qquad \mapsto \qquad w^{|w|}	 \in \set{a,b}^*.
\end{align*}
The automaton has two registers $r$ and $s$. Register $r$ will store words over the alphabet $\set{a,b}$ and register $s$ will store words over alphabet $\set{x}$, where $x$ is some variable symbol. Initially both registers are empty. 
When reading a letter $\sigma \in \set{a,b}$ the automaton does the following register update:
\begin{align*}
r:= r\sigma \qquad s:=sx	
\end{align*}
After it has finished reading the word, the automaton outputs $s[x \leftarrow r]$, i.e.~the contents of register $s$ with $r$ substituted for every occurrence of letter $x$.
\end{myexample} 

As seen in the above example, polynomial streaming transducers can have different alphabets for different registers, and a legitimate register operation is substitution. One has to be careful with substitution, however, since unrestricted use of substitution can yield  doubly exponential blowup. For example, if a register $r$ starts with value $xx$, and then we apply $n$ times the operation 
\begin{align*}
r := r[x \leftarrow r]	
\end{align*}
then the length of the final value will be the result of applying $n$ times the squaring operation $n \mapsto n^2$ to $2$, which is a number of doubly exponential size.  In the model below, we introduce a syntactic restriction which forbids this type of behaviour. Also, we allow regular lookahead (i.e.~the operation performed can also depend on some regular properties of the input that has not been read yet), and there will be a restriction on the way substitutions are used. 


\begin{definition}[Polynomial streaming transducer] The syntax of a polynomial streaming transducer consists of:
	\begin{itemize}
	\item input and output alphabets $\Sigma,\Gamma$;
		\item a totally ordered set of registers $R$;
		\item for each register $r \in R$, an associated alphabet $\Sigma_r$;
		\item a designated output register, with alphabet $\Gamma$.
		\item a rational transition function
\begin{align*}
  \delta : \Sigma^* \to  operations^*
\end{align*}
where the set of operations is:
\begin{align*}
  r := rs \qquad r:= sr \qquad r:=st \qquad r:= s[a \leftarrow t] \qquad r:=a
\end{align*}
such that $r,s,t \in R$ satisfy  $s<r$ and $t<r$ and $a \in \Sigma_r$.
	\end{itemize}
	The transducer is called \emph{first-order definable} if the transition function is such. The transducer is called \emph{linear} if it does not use substitution operations, i.e.~operations of the form $r:=s[a \leftarrow t]$.
\end{definition}
